DailyTalk: Spoken Dialogue Dataset for Conversational Text-to-Speech

The majority of current Text-to-Speech (TTS) datasets, which are collections of individual utterances, contain few conversational aspects. In this paper, we introduce DailyTalk, a high-quality conversational speech dataset designed for conversational TTS. We sampled, modified, and recorded 2,541 dialogues from the open-domain dialogue dataset DailyDialog inheriting its annotated attributes. On top of our dataset, we extend prior work as our baseline, where a non-autoregressive TTS is conditioned on historical information in a dialogue. From the baseline experiment with both general and our novel metrics, we show that DailyTalk can be used as a general TTS dataset, and more than that, our baseline can represent contextual information from DailyTalk. The DailyTalk dataset and baseline code are freely available for academic use with CC-BY-SA 4.0 license.

==> content/03_statistics.tex <==
% \subsection{Statistics}
% \label{sec:statistics}

% From the data collection procedure in section~\ref{sec:data_construction}, we collected recordings of 2,541 dialogues. In order to function as conversational TTS dataset, as mentioned above, \ours{} should function as both dialogue dataset and TTS dataset. In this section, we show statistics of \ours{} and compare them with existing TTS dataset and dialogue dataset to show sufficiency of our dataset as both aspects.

% \paragraph{\ours{} as a TTS dataset}
% In Table~\ref{tab:statistics_tts}, we show statistics of \ours{} while comparing with popular dataset for text-to-speech, LJSpeech \citep{ito2017ljspeech} and VCTK \citep{yamagishi2012vctk}. Our dataset has 

% \paragraph{Comparison with DailyDialog}
% Since data of \ours{} are randomly sampled from DailyDialog, script-related statistics of our dataset should follow that of DailyDialog. Our dataset has same category of emotion (anger, disgust, fear, joy, sadness, surprise, no emotion), topic (ordinary life, school life, culture \& education, attitude \& emotion, relationship, tourism, health, work, politics, finance), and dialogue act (inform, question, directive, commissive).  Figure~\ref{fig:stats1} shows comparison of statistical distribution between DailyDialog and \ours{}. As the histograms depict, \ours{} show similar distribution in terms of every aspect: emotion, topic and dialogue act. This result show that our dataset has diverse dialogues as well as DailyDialog dataset.

% \input{supplementary/statistics_phn_dt}
% \input{supplementary/phoneme_list}

% Table~\ref{tab:statistics_tts} shows detailed statistics of our dataset. \ours{} consists of 2,541 dialogues of 20 hours in total. We kept all the other script-related label distribution (e.g., emotion, dialog act, topic) derived from DailyDialog.

% Table~\ref{tab:statistics_tts} shows detailed statistics of our dataset. We also note per-speaker statistics so that one can refer when using the dataset of a single speaker. Phoneme distribution of \ours{} is provided in Figure~\ref{fig:phn_dt}, with comparison to the distributions of LJSpeech and VCTK. Phoneme distribution of each dataset is obtained by running open-sourced pretrained G2P model \cite{g2pE2019}\footnote{https://github.com/Kyubyong/g2p}. Included phonemes are listed in Table~\ref{tab:phoneme_list}. The order of phonemes in the table is same as x-axis of each distribution figure, from left to right. Our distribution contains a sufficient phonemes for successful TTS model training, except for some special phonemes that are rarely used in speeches.

% Expecting future expansion of our dataset, we design \ours{} to maintain the characteristics of DailyDialog. We randomly sampled scripts of \ours{} from DailyDialog, so that script-related statistics of our dataset follow DailyDialog. Our dataset has the same category of emotion (anger, disgust, fear, joy, sadness, surprise, no emotion), topic (ordinary life, school life, culture \& education, attitude \& emotion, relationship, tourism, health, work, politics, finance), and dialogue act (inform, question, directive, commissive). We also plot statistical distribution of \ours{}. Comparing to distributions of DailyDialog \cite{li2017dailydialog}, \ours{} show similar distribution in all aspects: emotion, topic and dialogue act. This result indicates that our dataset can be extended toward other instances in DailyDialog. 

% \input{supplementary/statistics_chr_dist}

==> content/06_related_works.tex <==
\section{Related Works}

% TTS data
Due to the amount of restriction for text-to-speech training data, there has been a limited amount of datasets constructed for neural TTS. One of the most popular and widely-used datasets is LJSpeech \cite{ito2017ljspeech}. Despite its contribution to the improvement of the neural TTS field, LJSpeech has a limitation in that it consists of only the reading style of a single speaker. Several speech corpora that mitigate such limitations exist, either increasing the number of speakers or adding more expressivity. LibriTTS \cite{zen2019libritts} and VCTK \cite{yamagishi2012vctk} are the multi-speaker speech corpora for text-to-speech, with large amount of speakers (>100). Blizzard Challenge \cite{king2013blizzard} consistently provides a high-quality dataset for expressive TTS by the annual challenge. Even several datasets and corpora provide high-quality data with various information, no open dataset exists that provides conversational information.

% Converational TTS
Recently, some studies in TTS have started to focus on conversational information to synthesize more dialogue-like speech. \cite{guo2021conversational} suggests an overall pipeline of conversational TTS, including data construction and neural network with consideration of dialogue history. This conversational TTS model has been improved either into more precise history modeling \cite{li2021spoken} or into a controllable network \cite{cong2021controllable}. Another interest exists in some research, which focuses on supplementary elements in conversation. \cite{yan2021adaspeech3} introduces AdaSpeech3, which models filling pauses in addition to speech synthesis. Even with improvements in various methods of representing conversations in TTS, the lack of an open dataset has been an obstacle, blocking easy access for people to conversational TTS studies.


==> content/a2_checklist.tex <==
% \section{Main Paper Checklist}

% \begin{enumerate}
% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{\bf We state limitation of our work in the Conclusion section. See Section~\ref{sec:conclusion}.} % Conclusion에 있음
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{\bf We discuss them in ethical considerations section. See section~\ref{sec:ethical_consideration}} % Ethical consideration 적자
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerNA{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerNA{}
% \end{enumerate}

% \item If you ran experiments (e.g. for benchmarks)...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{\bf }
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{\bf We described training details in Section~\ref{sec:experiments}.}
%   \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerNA{}
%   \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{\bf We used single RTX3090 GPU for training the baseline model. We include it in Section~\ref{sec:experiments}}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{} % no additional justification 
%   \item Did you mention the license of the assets?
%     \answerYes{\bf Our dataset is built upon DailyDialog dataset, which is publicly available for academic  use with CC-BY-SA 4.0 license. The license of our dataset is also notified in the instruction page\footnote{\url{https://github.com/keonlee9420/DailyTalk}}, abstract, and  Section~\ref{sec:data_construction}. See abstract and section~\ref{sec:data_construction}.}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerYes{\bf We included the dataset and baseline model URL.}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerYes{\bf Voice actors and crowdworkers are volunteered to this project. Also, we notified actors about the usage of dataset and obtained written agreement of usage.}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerYes{\bf We discuss personally identifiable information in ethical consideration section (Section~\ref{sec:ethical_consideration}). Our data does not contain any personally identifiable information but the voice, but actors agreed to distribute their voice as a dataset. Our dataset has no offensive content, since transcripts of our dataset are derived from existing DailyDialog dataset.}
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerYes{\bf We describe crowdsourcing details and instruction screenshot in Section~\ref{sec:experiments}.}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerYes{\bf We received IRB approval from KAIST (\#KH2021-227). We do not collect any personally identifiable information but the acting voice. We collected agreement of using recorded voice as a speech synthesis dataset.} 
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerYes{\bf The pre/post processing and recording of the dataset was conducted by crowdsourcing platforms, where all the workers were guaranteed minimum wage (about \$8 per hour). Total amount of spent is determined based on the duration of recording, which took about 40 hours.} 
% \end{enumerate}

% \end{enumerate}
